Reduction of the Beam Pointing Error for Improved Free-Space Optical Communication Link Performance

Free-space optical communication is emerging as a low-power, low-cost, and high data rate alternative to radio-frequency communication in short-to medium-range applications. However, it requires a close-to-line-of-sight link between the transmitter and the receiver. This paper proposes a robust $\cHi$ control law for free-space optical (FSO) beam pointing error systems under controlled weak turbulence conditions. The objective is to maintain the transmitter-receiver line, which means the center of the optical beam as close as possible to the center of the receiving aperture within a prescribed disturbance attenuation level. First, we derive an augmented nonlinear discrete-time model for pointing error loss due to misalignment caused by weak atmospheric turbulence. We then investigate the $\cHi$-norm optimization problem that guarantees the closed-loop pointing error is stable and ensures the prescribed weak disturbance attenuation. Furthermore, we evaluate the closed-loop outage probability error and bit error rate (BER) that quantify the free-space optical communication performance in fading channels. Finally, the paper concludes with a numerical simulation of the proposed approach to the FSO link's error performance.

==> README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> arxiv-style-master IFAC Journal Submitted/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> arxiv-style-master IFAC Journal Submitted/setup-IEEEtrans.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%      setup pour articles     %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%% reglages des flottants %%%%%%%%%%%%%%%%%%%%
\renewcommand{\floatpagefraction}{.95} % les flottants peuvent occuper
% 95% de la page
\renewcommand{\textfraction}{.1} % le texte peut n'occuper que 10% de
% la page
\renewcommand{\dblfloatpagefraction}{.99} % les flottants en twocolumn
% peuvent occuper 90% de la page
\renewcommand{\dbltopfraction}{0.90} % 90% du top peut etre occup� par
% les flottants en twocolumn
\renewcommand{\dblfloatsep}{0pt} % espace entre flottants et d�but/fin
% de la page en twocolumn
\renewcommand{\dbltextfloatsep}{0pt} % espace entre flottants du d�but/fin
% de la page et texte en twocolumn
\renewcommand{\intextsep}{0pt} % espace vertical entre flottants et
% texte en twocolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% modification de l'interligne (80% de l'original)
% \renewcommand{\baselinestretch}{.8}

% To adjust the position of the text on the page
% (for our specific printer) with the commands
%            \addtolength{\oddsidemargin}{Xmm} % right Xmm
%           \addtolength{\topmargin}{Ymm}     % down Ymm

% \addtolength{\topmargin}{10mm} %rajoute 1 cm en haut de la page

% \setlength{\labelsep}{1pt}
% \setlength{\itemsep}{0pt}

% espaces dans les tableaux
\renewcommand{\arraystretch}{1.3} % diminue hauteur des lignes dans tableaux
% \setlength{\arraycolsep}{1pt}
\setlength{\arraycolsep}{5pt} % espace entre les colonnes (array et matrix)
\setlength{\tabcolsep}{1pt}
% \addtolength{\doublerulesep}{-1pt} % espace entre double trait
% \addtolength{\extratabsurround}{-2pt}

%% listes compactes avec mdwlist
%\makecompactlist{enumerateb}{enumerate}
%\makecompactlist{itemizeb}{itemize}
%\makecompactlist{descriptionb}{description}

\allowdisplaybreaks % Autorise la coupure de fin de page

% red�finition des tailles exposants/indices maths %%change HS 15-05-2001
% \DeclareMathSizes{12}{12}{7}{5}
% \DeclareMathSizes{11}{11}{7}{5}
% \DeclareMathSizes{10}{9}{6}{4}

% Spaces before and after environment EQ
\setlength{\abovedisplayskip}{1 mm}
\setlength{\belowdisplayskip}{1 mm}
\setlength{\abovedisplayshortskip}{1 mm}
\setlength{\belowdisplayshortskip}{1 mm}

% Affiche des numeros jusq'au paragraph
\setcounter{secnumdepth}{4}
% profondeur de la toc
\setcounter{tocdepth}{4} % jusqu'a sous-section
% profondeur de la lof
% \setcounter{lofdepth}{3} % jusqu'a caption "x.a", "x.b"

% rajoute de la hauteur de page
% \addtolength{\textheight}{0.2in}
% \addtolength{\headsep}{-2mm}

% permet une num�rotation des �quations en rapport avec la section
% \numberwithin{equation}{section}
% \numberwithin{newenvironment}{section}

% permet une sous-num�rotation en lettres dans subequations et
% subeqnarray
% \def\theequation{\alph{equation}}
% \def\thesubequation{\theequation\alph{subequation}}
% \renewcommand{\theequation}{\theparentequation\alph{equation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Attention -- ancienne version --
% permet une sous-num�rotation en lettres dans subequations
% � inserer � l'int�rieur de l'environnement subequations
% \renewcommand{\thesubequation}{\theequation\alph{subequation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%% Red�finition des sections
% \def\thesection {\arabic{section}.}
% \def\thesubsection {\thesection\arabic{subsection}.}
% \def\thesubsubsection {\thesubsection\arabic{subsubsection}.}
% \def\theparagraph {\thesubsubsection\arabic{paragraph}.}
% \def\thesubparagraph {\theparagraph\arabic{subparagraph}.}

% permet une �num�ration (i),(ii),(iii)
% \def\labelenumi{(\bf\theenumi)}     \def\theenumi{\roman{enumi}}
% \def\labelenumii{\bf\theenumii}  \def\theenumii{$\scriptstyle\bullet$}
% \def\labelenumiii{\theenumiii.} \def\theenumiii{\arabic{enumiii}}
% \def\labelenumiv{\theenumiv.}   \def\theenumiv{\alph{enumiv}}
% \def\p@enumii{\theenumi}
% \def\p@enumiii{\theenumi(\theenumii)}
% \def\p@enumiv{\p@enumiii\theenumiii}

% D�finition de la date du jour en Fran�ais
\def\aujour{\number\day \space \ifcase\month\or
janvier\or f�vrier\or mars\or avril\or mai\or
juin\or juillet\or ao�t\or septembre\or octobre\or
novembre\or d�cembre\fi \space \number\year}

% diff�rents espaces verticaux sans indentations apr�s
\newcommand{\petesp}{{\smallskip \noindent}}
\newcommand{\moyesp}{{\medskip \noindent}}
\newcommand{\graesp}{{\bigskip \noindent}}
\newcommand{\ggraesp}{{\bigskip \bigskip \noindent}}

\newcommand{\nid}{{\noindent}}

% en gras
\def\bA{{\bf A}}
\def\bB{{\bf B}}
\def\bC{{\bf C}}
\def\bD{{\bf D}}
\def\bBu{{{\bf B}_u}}
\def\bBw{{{\bf B}_w}}
\def\bCy{{{\bf C}_y}}
\def\bDyu{{{\bf D}_{yu}}}
\def\bDyw{{{\bf D}_{yw}}}
\def\bCz{{{\bf C}_z}}
\def\bDzu{{{\bf D}_{zu}}}
\def\bDzw{{{\bf D}_{zw}}}
\def\bE{{\bf E}}
\def\bF{{\bf F}}
\def\bG{{\bf G}}
\def\bH{{\bf H}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bK{{\bf K}}
\def\bL{{\bf L}}
\def\bM{{\bf M}}
\def\bN{{\bf N}}
\def\bO{{\bf O}}
\def\bP{{\bf P}}
\def\bQ{{\bf Q}}
\def\bR{{\bf R}}
\def\bS{{\bf S}}
\def\bT{{\bf T}}
\def\bU{{\bf U}}
\def\bV{{\bf V}}
\def\bW{{\bf W}}
\def\bX{{\bf X}}
\def\bY{{\bf Y}}
\def\bZ{{\bf Z}}

% en calligraphi�
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

\def\cIr{{\cal I}(r)}
\def\cSr{{\cal S}(r)}
\def\cBr{{\cal B}(r)}
\def\cDr{{\cal D}(r)}
\def\cGr{{\cal G}(r)}
\def\cFl{{\cal F}_{l}}
\def\cFu{{\cal F}_{u}}
\def\cEP{\mbox{${\cal E}_P$}}
\def\cEQinv{\mbox{${\cal E}_{Q^{-1}}$}}

% widetilde
\def\tA{{\widetilde{A}}}
\def\tB{{\widetilde{B}}}
\def\tC{{\widetilde{C}}}
\def\tD{{\widetilde{D}}}
\def\tE{{\widetilde{E}}}
\def\tF{{\widetilde{F}}}
\def\tG{{\widetilde{G}}}
\def\tH{{\widetilde{H}}}
\def\tI{{\widetilde{I}}}
\def\tJ{{\widetilde{J}}}
\def\tK{{\widetilde{K}}}
\def\tL{{\widetilde{L}}}
\def\tM{{\widetilde{M}}}
\def\tN{{\widetilde{N}}}
\def\tO{{\widetilde{O}}}
\def\tP{{\widetilde{P}}}
\def\tQ{{\widetilde{Q}}}
\def\tR{{\widetilde{R}}}
\def\tS{{\widetilde{S}}}
\def\tT{{\widetilde{T}}}
\def\tU{{\widetilde{U}}}
\def\tV{{\widetilde{V}}}
\def\tW{{\widetilde{W}}}
\def\tX{{\widetilde{X}}}
\def\tY{{\widetilde{Y}}}
\def\tZ{{\widetilde{Z}}}
\def\tek{{\widetilde{e}}_k}
\def\tr{{\widetilde{r}}}
\def\tx{{\widetilde{x}}}

% overline
\def\oA{{\overline{A}}}
\def\oB{{\overline{B}}}
\def\oC{{\overline{C}}}
\def\oD{{\overline{D}}}
\def\oE{{\overline{E}}}
\def\oF{{\overline{F}}}
\def\oG{{\overline{G}}}
\def\oH{{\overline{H}}}
\def\oI{{\overline{I}}}
\def\oJ{{\overline{J}}}
\def\oK{{\overline{K}}}
\def\oL{{\overline{L}}}
\def\oM{{\overline{M}}}
\def\oN{{\overline{N}}}
\def\oO{{\overline{O}}}
\def\oP{{\overline{P}}}
\def\oQ{{\overline{Q}}}
\def\oR{{\overline{R}}}
\def\oS{{\overline{S}}}
\def\oT{{\overline{T}}}
\def\oU{{\overline{U}}}
\def\oV{{\overline{V}}}
\def\oW{{\overline{W}}}
\def\oX{{\overline{X}}}
\def\oY{{\overline{Y}}}
\def\oZ{{\overline{Z}}}
\def\ova{{\overline{a}}}
\def\ovb{{\overline{b}}}
\def\ovx{{\overline{x}}}
\def\ovg{{\overline{g}}}
\def\ovr{{\overline{r}}}

% widehat
\def\hA{{\widehat{A}}}
\def\hB{{\widehat{B}}}
\def\hC{{\widehat{C}}}
\def\hD{{\widehat{D}}}
\def\hE{{\widehat{E}}}
\def\hF{{\widehat{F}}}
\def\hG{{\widehat{G}}}
\def\hH{{\widehat{H}}}
\def\hI{{\widehat{I}}}
\def\hJ{{\widehat{J}}}
\def\hK{{\widehat{K}}}
\def\hL{{\widehat{L}}}
\def\hM{{\widehat{M}}}
\def\hN{{\widehat{N}}}
\def\hO{{\widehat{O}}}
\def\hP{{\widehat{P}}}
\def\hQ{{\widehat{Q}}}
\def\hR{{\widehat{R}}}
\def\hS{{\widehat{S}}}
\def\hT{{\widehat{T}}}
\def\hU{{\widehat{U}}}
\def\hV{{\widehat{V}}}
\def\hW{{\widehat{W}}}
\def\hX{{\widehat{X}}}
\def\hY{{\widehat{Y}}}
\def\hZ{{\widehat{Z}}}
\def\whx{{\widehat{x}}} % MZ
\def\whw{{\widehat{w}}} % MZ
\def\whz{{\widehat{z}}} % MZ

% orthogonaux
\def\orthU{{U_{\rm orth}}}
\def\orthV{{V_{\rm orth}}}
\def\pU{{U_{\perp}}}
\def\pV{{V_{\perp}}}
\def\torthU{{\tilde{U}_{\rm orth}}}
\def\torthV{{\tilde{V}_{\rm orth}}}

% math environnements
% \def\BA[{\left[\begin{array}} % a revoir
% \def\BEAS{\begin{eqnarray*}} % a revoir
% \def\BEA{\begin{eqnarray}} % a revoir
% \def\BEQ{\begin{equation}} % a revoir
% \def\Co{{\mathop {\bf Co}}} % a revoir
% \def\EA]{\end{array}\right]} % a revoir
% \def\EEAS{\end{eqnarray*}} % a revoir
% \def\EEA{\end{eqnarray}} % a revoir
% \def\EEQ{\end{equation}} % a revoir
% \newcommand{\EEL}[1]{\label{#1}\end{equation}} % a revoir

% New environments thms, etc
% \theoremstyle{plain} % avec num�rotation relative selon les sections
% \newtheorem{thm}{Theorem}[section]
% \newtheorem{cor}[thm]{Corollary}
% \newtheorem{prop}[thm]{Proposition}
% \newtheorem{lemma}[thm]{Lemma}
% \newtheorem{proper}[thm]{Property}
%\newtheorem{defi}[thm]{Definition}
% \newtheorem{prob}[thm]%{Problem}

% % \theoremstyle{definition}
% % \newtheorem{defi}{Definition}[section]

% \theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\newtheorem{ass}{Assumption}
%\newtheorem{lemma}{Lemma}
%\newtheorem{col}{Corollary}
%\newtheorem{theorem}{Theorem}
\newtheorem{thm}{Theorem}
%\newtheorem{defi}{Definition}
\newtheorem{proof}{Proof}
% \theoremstyle{algo}
% \newtheorem{algo}[thm]{Algorithm}%{Algorithme}

% \newass{ass}{Assumption}
%
% % avec ou sans num�rotation selon les section et non relative
% \theoremstyle{plain}
% \newtheorem{defi}{Definition}%{D�finition}%[section]
% \newtheorem{lemma}{Lemma}%{Lemme}%[section]
% \newtheorem{cor}{Corollary}%{Corollaire}%[section]
% \newtheorem{thm}{Theorem}%{Th�or�me}%[section]
% \newtheorem{prop}{Proposition}%{Proposition}%[section]
%  % \newtheorem{ass}{Assumption}%{Hypoth�se}%[section]
% \newtheorem{proper}{Property}%{Propri�t�}%[section]
% \newtheorem{prob}{Problem}%{Probl�me}%[section]

%\newtheorem{thm}{Theorem}%{Th\'eor\`eme}%{Th�or�me}%[section]
%% \newtheorem{defi}{Definition}%{D�finition}%[section]
%\newtheorem{lem}{Lemma}%{Lemme}%[section]
%\newtheorem{col}{Corollary}%{Corollaire}%{Corollary}%{Corollaire}%[section]
%\newtheorem{prop}{Proposition}%{Proposition}%[section]
%% \newtheorem{ass}{Assumption}%{Hypoth�se}%[section]
%\newtheorem{proper}{Property}%{Propri�t�}%[section]
%% \newtheorem{prob}{Problem}%{Probl�me}%[section]
%% \newtheorem*{prob*}{Problem} % sans numeotation (amsthm)
%%\newtheorem{proo}{Proof}%{Probl�me}%[section]
%% \theoremstyle{remark} % corps en caract�res droit
%% \newtheorem{remark}{Remark}%{Remarque}%[section]

%\theoremstyle{definition}
%\newtheorem{defi}{Definition} %{D�finition}%[section]
%\newtheorem{prob}{Problem} %{Probl�me}%[section]
%\newtheorem*{prob*}{Problem} % sans numerotation (amsthm)
%\newtheorem{remark}{Remarque}%{Remark} %{Remarque}%[section]
%\newtheorem*{remark*}{Remark} % sans numerotation (amsthm)
%\newtheorem{ass}{Assumption}%{Hypoth\`ese}%{Assumption}%{Hypoth�se}%[section]
%%\newtheorem{proo}{Proof}
%% \theoremstyle{algo}
%\newtheorem{algo}{Algorithm}%{Algorithme}%[chapter]

\newcommand{\ethm}{\ding{110}}%charact�re fin_de_th�or�me
\newcommand{\elem}{$\square$}%charact�re fin_de_lemme
\newcommand{\edefini}{\ding{117}}%charact�re fin_de_d�finition
\newcommand{\eass}{\ding{114}}%charact�re fin_d'assumption
\newcommand{\ermk}{\ding{113}}%charact�re fin_de_remarque
\newcommand{\eprop}{\ding{109}}%charact�re fin_de_proposition

% \renewcommand{\qedsymbol}{\ding{111}}
%\renewcommand{\qedsymbol}{$\large\bullet$}

\newcommand{\units}[2]{#1\textrm{\thinspace \thinspace #2}} %unit�s de mesure

% d�finitions des ensembles Math�matiques
%%% Cr�ations EM
\def\C{{\setbox0=\hbox{$\displaystyle{\rm C}$}
        \hbox{\hbox to0pt{\kern 0.4\wd0\vrule height 0.95\ht0\hss}\box0}}}
        % ensemble des Complexes --> OK
\def\Q{{\setbox0=\hbox{$\displaystyle{\rm Q}$}%
    \hbox{\raise 0.2\ht0\hbox to0pt{\kern 0.4\wd0\vrule height
    0.85\ht0\hss}\box0}}} % ensemble des Rationnels --> � revoir
\def\R{\mathop{\rm I\mkern -3.5mu R}} % ensemble des R�els --> OK
\def\N{\mathop{\rm I\mkern -3.5mu N}} % ensemble des Entiers --> OK
\def\Cij{{\C}^{i\times j}}
\def\Cn{{\C}^n}
\def\Rij{{\R}^{i\times j}}
\def\Rj{{\R}^j}
\def\Rji{{\R}^{j\times i}}
\def\Rjrmi{{\R}^{(j+r)\times (m+i)}}
\def\Rjrnur{{\R}^{(j+r)\times (n_{1}+r)}}
\def\Rk{{\R}^k}
\def\Rki{{\R}^{k_{i}}}
\def\Rkk{{\R}^{k\times k}}
\def\Rokok{{\R}^{\overline{k}\times \overline{k}}}
\def\Rkiki{{\R}^{k_{i}\times k_{i}}}
\def\Rkl{{\R}^{(k+\ell)}}
\def\Rklkl{{\R}^{(k+\ell)\times (k+\ell)}}
\def\Rksiksi{{\R}^{k_{s+i}\times k_{s+i}}}
\def\Rell{{\R}^{\ell}}
\def\Rm{{\R}^m}
\def\Rmone{{\R}^{m_{1}}}
\def\Rmtwo{{\R}^{m_{2}}}
\def\Rmoneone{{\R}^{m_{1}\times m_{1}}}
\def\Rmtwotwo{{\R}^{m_{2}\times m_{2}}}
\def\Rmn{{\R}^{m\times n}}
\def\Rmq{{\R}^{m\times q}}
\def\Rn{{\R}^n}
\def\Rden{{\R}^{2n}}
\def\Rnone{{\R}^{n_{1}}}
\def\Rntwo{{\R}^{n_{2}}}
\def\Rnk{{\R}^{n+k}}
\def\Rnm{{\R}^{n\times m}}
\def\Rnmnm{{\R}^{(n+m)\times (n+m)}}
\def\Rnurmi{{\R}^{(n_{1}+r)\times (m+i)}}
\def\Rnn{{\R}^{n\times n}}
\def\RNN{{\R}^{N\times N}}
\def\Rnnu{{\R}^{n\times n_{u}}}
\def\Rnunu{{\R}^{n_{1}\times n_{1}}}
\def\Rnurnur{{\R}^{(n_{1}+r)\times (n_{1}+r)}}
\def\Rnnw{{\R}^{n\times n_{w}}}
\def\Rnny{{\R}^{n\times n_{y}}}
\def\Rnp{{\R}^{n\times p}}
\def\Rnpp{{\R}^{n-p}}
\def\Rnpn{{\R}^{(n-p)\times n}}
\def\Rnurdp{{\R}^{(n_{1}+r)\times 2p}}
\def\Rnrnr{{\R}^{(n+r)\times (n+r)}}
\def\Rnq{{\R}^{n\times q}}
\def\Rnr{{\R}^{n\times r}}
\def\Rp{{\R}^p}
\def\Rpone{{\R}^{p_{1}}}
\def\Rptwo{{\R}^{p_{2}}}
\def\Rpn{{\R}^{p\times n}}
\def\Rpq{{\R}^{p\times q}}
\def\Rdpmi{{\R}^{2p\times (m+i)}}
\def\Rdpnur{{\R}^{2p\times (n_{1}+r)}}
\def\Rponeone{{\R}^{p_{1}\times p_{1}}}
\def\Rptwotwo{{\R}^{p_{2}\times p_{2}}}
\def\Rq{{\R}^q}
\def\Rqone{{\R}^{q_{1}}}
\def\Rqtwo{{\R}^{q_{2}}}
\def\Rqq{{\R}^{q\times q}}
\def\Rqoneone{{\R}^{q_{1}\times q_{1}}}
\def\Rqtwotwo{{\R}^{q_{2}\times q_{2}}}
\def\Rr{{\R}^r}
\def\Rrone{{\R}^{r_{1}}}
\def\Rrtwo{{\R}^{r_{2}}}
\def\Rrn{{\R}^{r\times n}}
\def\Rrp{{\R}^{r\times p}}
\def\Rrdp{{\R}^{r\times 2p}}
\def\Rrr{{\R}^{r\times r}}
\def\Rs{{\R}^s}
\def\Rv{{\R}^v}
\def\Rvone{{\R}^{v_{1}}}
\def\Rvtwo{{\R}^{v_{2}}}
\def\Rvv{{\R}^{v\times v}}
%% versions newsgroup "fr.comp.text.tex"
\def \ensN {\mbox{I\hspace{-.15em}N}}
\def \ensR {\mbox{I\hspace{-.15em}R}}
\def \ensZ {\mbox{Z\hspace{-.32em}Z}}
\def \ensC {\mbox{l\hspace{-.47em}C}}
\def \ensQ {\mbox{l\hspace{-.47em}Q}}
% autre d�finition de Z et de N
% \newcommand{\Z}{$\Bbb Z$}                 % D�finition du Z math�matique
% \newcommand{\N}{{\it I\!\!N}}             % D�finition du N math�matique
% \newcommand{\ZZ}{\mathbb{Z}}              % D�finition du Z math�matique
% \newcommand{\NN}{\mathbb{N}}              % D�finition du N math�matique

% math symbols and operators
\def\Expect{\mathop{\bf E}} % esp�rance

% \def\cHi{\mathop{{\mathcal{H}}_{\infty}} % Hinf calligraphi� (norme)
% \def\cH2{\mathop{{\mathcal{H}}_2} % H2 calligraphi� (norme)
\def\cHi{{\cal H}_{\infty}} % Hinf calligraphi� (norme)
\def\cH2{{\cal H}_2} % H2 calligraphi� (norme)
\def\cU{{\cal U}}

\def\cLi{\mathop{\mathcal L}_{\infty}} % Linf
\def\cLone{\mathop{\mathcal L}_{1}} % L1
\def\cL2{\mathop{\mathcal L}_{2}} % espace carr�-int�grable
%en continu
\def\cHinfc{{\cal H}_{\infty}^c} % espace Banach pour continu
\def\cHtwoc{{\cal H}_2^c} % espace Hilbert pour continu
%en discret
\def\cHinfd{{\cal H}_{\infty}^d} % espace Banach pour discret
\def\cHtwod{{\cal H}_2^d} % espace Hilbert pour discret

\def\cRHi{\mathop{\cal R \cal H}_\infty} % RHinf calligraphi� (norme)
\def\cRH2{\mathop{\cal R \cal H}_2} % RH2 calligraphi� (norme)
\def\cRLi{\mathop{\cal R \cal L}_{\infty}} % RLinf
\def\cRLone{\mathop{\cal R \cal L}_{1}} % RL1
\def\cRL2{\mathop{\cal R \cal L}_{2}} % espace carr�-int�grable

\def\Ltwo{{\bf L}_2}

% \def\Reel{\mbox{\bf Re}}
% \def\Im{\mbox{\bf Im}}
%
% \def\log{\mbox{\bf log}}
% \def\det{\mbox{\bf det}}
% \def\rank{\mbox{\bf rank}}
% \def\tra{\mathop{\bf tr}}
% \def\diag{\mbox{\bf diag}}
% \def\bdiag{\mbox{\bf bdiag}}
% \def\herm{\mbox{\bf herm}}
% \def\ker{\mbox{\bf ker}}
% \def\image{\mbox{\bf span}}
% \def\cond{\mbox{\bf cond}}
% \def\min{\mbox{\bf min}}
% \def\max{\mbox{\bf max}}
% \def\dim{\mbox{\bf dim}}
% \def\deg{\mbox{\bf deg}}
% \def\exp{\mbox{\bf exp}}
% \def\lim{\mbox{\bf lim}}

\def\Prob{\mathop{\bf Prob}}

% \def\Reel{\mbox{Re}}
% \def\Im{\mbox{Im}}
%
% \def\det{\mbox{det}}
% \def\rank{\mbox{rank}}
% \def\tra{\mathop{tr}}
% \def\diag{\mbox{diag}}
% \def\bdiag{\mbox{bdiag}}
% \def\herm{\mbox{herm}}
% \def\ker{\mbox{ker}}
% \def\image{\mbox{span}}
% \def\cond{\mbox{cond}}
% \def\min{\mbox{min}}
% \def\max{\mbox{max}}
% \def\dim{\mbox{dim}}
% \def\deg{\mbox{deg}}
% \def\exp{\mbox{exp}}
% \def\lim{\mbox{lim}}
\DeclareMathOperator*{\bdiag}{bdiag}
\DeclareMathOperator*{\dcond}{cond}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\esp}{Esp}
\DeclareMathOperator*{\herm}{herm}
\DeclareMathOperator*{\im}{Im}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\re}{Re}
\DeclareMathOperator*{\sgn}{sgn}
% \DeclareMathOperator*{\span}{span}
\DeclareMathOperator*{\trace}{tr}
\DeclareMathOperator*{\vect}{vect}
\DeclareMathOperator*{\vectb}{vectb}
\def\vectbc{\mbox{vectb}_{\textrm{c}}}
\def\vectbr{\mbox{vectb}_{\textrm{r}}}
\DeclareMathOperator*{\with}{with}
\DeclareMathOperator*{\der}{d}
\DeclareMathOperator*{\Sym}{Sym}
\DeclareMathOperator*{\spec}{spec}
\DeclareMathOperator*{\eig}{eig}

% fonction de normes, abs, norme Hinf, norme H2, norm Linf et norme L2
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\norminf}[1]{{\left\|{#1}\right\|}_{\infty}}
\newcommand{\normtwo}[1]{{\left\|{#1}\right\|}_{2}}
\newcommand{\normLinf}[1]{{\left\|{#1}\right\|}_{{\cal L}_{\infty}}}
\newcommand{\normLtwo}[1]{{\left\|{#1}\right\|}_{{\cal L}_{2}}}

% double overline
\newcommand{\bbar}[1]{\overline{\overline{#1}}}

% regular height vertical bar
\def\setmid{\, \mid \,}
% scalable vertical bar (must be paired with \right.)
\def\leftsetmid{ \; \left| \; }
% scalable vertical bar (must be paired with \left.)
\def\rightsetmid{ \; \right| \; }

%\renewcommand{\QED}{\textbullet}
%\def\QED{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
\def\qedsymbol{\textbullet}
%\renewcommand{\proofname}{Proof}
%\def\TheWordProof{D�monstration\enskip}

\def\SAT{\mbox{SAT}}
\def\SD{\mbox{SD}}

%\def\approxeq{\approx}
%\def\approxleq{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}
%{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\def\argmin{\mathop{\rm argmin}}
\def\eqbydef{\mathrel{\stackrel{\Delta}{=}}}
\def\infeqyn{\mathrel{\stackrel{{\large ?}}{\leqslant}}}
\def\supeqyn{\mathrel{\stackrel{{\large ?}}{\geqslant}}}

\def\mini{\mathop{\min}} % � utiliser avec par exemple
% "\underset{X\in\Phi}{\mini}\; V(X)"
\def\maxi{\mathop{\max}} % � utiliser avec par exemple
% "\underset{X\in\Phi}{\maxi}\; V(X)"
\def\limi{\mathop{\lim}}

%\newcommand{\mina}[1]{\mathrel{\stackrel{\min}{#1}}}
%\newcommand{\maxa}[1]{\mathrel{\stackrel{\max}{#1}}}
% � utiliser avec \mina{xxx} ou bien maxa{xxx}

%\newcommand{\sigmaM}{{\ensuremath{\sigma_{\max}}}}
\newcommand{\sigmaM}{\ensuremath{\overline{\sigma}}}
%\newcommand{\sigmam}{\ensuremath{\sigma_{\min}}}
\newcommand{\sigmam}{\ensuremath{\underline{\sigma}}}
\newcommand{\lambdaM}{\ensuremath{\lambda_{\rm max}}}
\newcommand{\lambdam}{\ensuremath{\lambda_{\rm min}}}
\def\argmax{{\mbox{argmax}}}
\def\lambdaopt{\lambda^{\rm opt}}

\def\xst{{x^{*}}}
\def\xopt{{x^{\rm opt}}}
\def\lambdak{{\lambda^{(k)}}}
\def\lambdakp{{\lambda^{(k+1)}}}

\def\Aaug{A_{\rm aug}}
\def\Baug{B_{\rm aug}}
\def\Bpaug{B_{{\rm aug},\, p}}
\def\Bwaug{B_{{\rm aug},\, w}}
\def\Cqaug{C_{{\rm aug},\,q}}
\def\Dqpaug{D_{{\rm aug},\, qp}}
\def\Czaug{C_{{\rm aug},\,z}}
\def\xaug{x_{\rm aug}}
\def\Paug{P_{\rm aug}}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\nd}[1]{${#1}^{\textrm{nd}}$}
\newcommand{\st}[1]{${#1}^{\textrm{st}}$}
\newcommand{\thh}[1]{${#1}^{\textrm{th}}$}
\newcommand{\rd}[1]{${#1}^{\textrm{rd}}$}
\newcommand{\eme}[1]{${#1}^{\textrm{\`eme}}$}
\newcommand{\ere}[1]{${#1}^{\textrm{\`ere}}$}
\newcommand{\er}[1]{${#1}^{\textrm{er}}$}
\newcommand{\eal}{{\it et al.\ }}
%\newcommand{\eqref}[1]{\mbox{(\ref{#1})}}
%\newcommand{\frgui}[1]{``{#1}''} % french guillemets --> OK
\newcommand{\frgui}[1]{`{#1}'}
\newcommand{\frguib}[1]{``{#1}''}

\newcommand{\dis}[1]{\displaystyle{#1}}
% espace top et bottom dans ligne de array% a utiliser avec \Ts et \Bs
\newcommand\setTBstruts{\def\Ts{\rule{0pt}{2.6ex}}%
                        \def\Bs{\rule[-1.2ex]{0pt}{0pt}}}

\newcommand{\XXX}[1]{\marginpar{\raggedright \footnotesize #1}}

% nom du label pour figures : Fig.
% \renewcommand\figurename{fig.}
%
% \renewcommand\tablename{\textbf{tab.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sfrac : ecrire proprement a/b
\makeatletter
\DeclareRobustCommand\sfrac[1]{\@ifnextchar/{\@sfrac{#1}}
                                            {\@sfrac{#1}/}}
\def\@sfrac#1/#2{\leavevmode\kern.1em\raise.5ex
         \hbox{$\m@th\fontsize\sf@size\z@
                           \selectfont#1$}\kern-.1em
         /\kern-.15em\lower.25ex
          \hbox{$\m@th\fontsize\sf@size\z@
                            \selectfont#2$}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% plotting command
\newcommand{\mplot}[4]{
    \begin{figure}[ftb]
    \begin{center}
    \unitlength 0.30 truein
    \begin{picture}(10,10)(6,6.5)
    \special{psfile = #1.ps hscale=70 vscale=70}
    \put(10,6.4){#3}
    \put(.5,13){#4}
    \end{picture}
    \caption{#2}
    \label{fig:#1}
    \end{center}
    \end{figure}
}

\newcommand{\mplotm}[4]{
    \begin{figure}[ftb]
    \begin{center}
    \unitlength 0.15 truein
    \begin{picture}(10,12)(6,6.5)
    \special{psfile = #1.ps hscale=35 vscale=35}
    \put(10,6.1){{\small #3}}
    \put(.5,13){{\small #4}}
    \end{picture}
    \caption{#2}
    \label{fig:#1}
    \end{center}
    \end{figure}
}

\newcommand{\mplotlr}[7]{
\begin{figure}[ftb]
     \unitlength 0.15 truein
     \begin{picture}(10,12)(6,6.5)
           \put(5,0){\special{psfile = #1.ps hscale=35 vscale=35}}
           \put(15,6.1){{\small #3}}
       \put(5.5,13){{\small #4}}
           \put(25,0){\special{psfile = #5.ps hscale=35 vscale=35}}
           \put(35,6.1){{\small #6}}
       \put(25.5,13){{\small #7}}
     \end{picture}
\caption{#2}
\label{fig:#1}
\end{figure}
}

